Stable Geodesic Update on Hyperbolic Space and its Application to Poincare Embeddings

A hyperbolic space has been shown to be more capable of modeling complex networks than a Euclidean space. This paper proposes an explicit update rule along geodesics in a hyperbolic space. The convergence of our algorithm is theoretically guaranteed, and the convergence rate is better than the conventional Euclidean gradient descent algorithm. Moreover, our algorithm avoids the "bias" problem of existing methods using the Riemannian gradient. Experimental results demonstrate the good performance of our algorithm in the \Poincare embeddings of knowledge base data.

==> 02_title_author.tex <==
\title{Geodesic Update on Hyperbolic Space and  its Application to \Poincare Embeddings}
% \titlenote{Produces the permission block, and
%   copyright information}
% \subtitle{Extended Abstract}
% \subtitlenote{The full version is available at  \texttt{acmart.pdf} document}


\author{Yosuke Enokida}
% \authornote{Equal contribution}
% \orcid{1234-5678-9012}
\affiliation{%
  \institution{The University of Tokyo}
%   \streetaddress{P.O. Box 1212}
  \city{Tokyo}
  \country{Japan}
%   \postcode{43017-6221}
}
\email{trovato@corporation.com}

\author{Atsushi Suzuki}
% \authornote{Equal contribution}
% \orcid{1234-5678-9012}
\affiliation{%
  \institution{The University of Tokyo}
%   \streetaddress{P.O. Box 1212}
  \city{Tokyo}
  \country{Japan}
%   \postcode{43017-6221}
}
\email{atsushi.suzuki.rd@gmail.com}

\author{Kenji Yamanishi}
% \authornote{Equal contribution}
% \orcid{1234-5678-9012}
\affiliation{%
  \institution{The University of Tokyo}
%   \streetaddress{P.O. Box 1212}
  \city{Tokyo}
  \country{Japan}
%   \postcode{43017-6221}
}
\email{yamanishi@mist.i.u-tokyo.ac.jp}

% \author{Valerie B\'eranger}
% \affiliation{%
%   \institution{Inria Paris-Rocquencourt}
%   \city{Rocquencourt}
%   \country{France}
% }
% \author{Aparna Patel}
% \affiliation{%
%  \institution{Rajiv Gandhi University}
%  \streetaddress{Rono-Hills}
%  \city{Doimukh}
%  \state{Arunachal Pradesh}
%  \country{India}}
% \author{Huifen Chan}
% \affiliation{%
%   \institution{Tsinghua University}
%   \streetaddress{30 Shuangqing Rd}
%   \city{Haidian Qu}
%   \state{Beijing Shi}
%   \country{China}
% }

% \author{Charles Palmer}
% \affiliation{%
%   \institution{Palmer Research Laboratories}
%   \streetaddress{8600 Datapoint Drive}
%   \city{San Antonio}
%   \state{Texas}
%   \postcode{78229}}
% \email{cpalmer@prl.com}

% \author{John Smith}
% \affiliation{\institution{The Th{\o}rv{\"a}ld Group}}
% \email{jsmith@affiliation.org}

% \author{Julius P.~Kumquat}
% \affiliation{\institution{The Kumquat Consortium}}
% \email{jpkumquat@consortium.net}

% % The default list of authors is too long for headers.
% \renewcommand{\shortauthors}{Y. Enokida et al.}













% \twocolumn[

% \icmltitle{Geodesic Update on Hyperbolic Space and  its Application to \Poincare Embeddings}

% % It is OKAY to include author information, even for blind
% % submissions: the style file will automatically remove it for you
% % unless you've provided the [accepted] option to the icml2018
% % package.

% % List of affiliations: The first argument should be a (short)
% % identifier you will use later to specify author affiliations
% % Academic affiliations should list Department, University, City, Region, Country
% % Industry affiliations should list Company, City, Region, Country

% % You can specify symbols, otherwise they are numbered in order.
% % Ideally, you should not use this facility. Affiliations will be numbered
% % in order of appearance and this is the preferred way.
% \icmlsetsymbol{equal}{*}

% \begin{icmlauthorlist}
% \icmlauthor{Yosuke Enokida}{ut}
% \icmlauthor{Atsushi Suzuki}{ut}
% \icmlauthor{Kenji Yamanishi}{ut}
% % \icmlauthor{Aeiau Zzzz}{equal,to}
% % \icmlauthor{Bauiu C.~Yyyy}{equal,to,goo}
% % \icmlauthor{Cieua Vvvvv}{goo}
% % \icmlauthor{Iaesut Saoeu}{ed}
% % \icmlauthor{Fiuea Rrrr}{to}
% % \icmlauthor{Tateu H.~Yasehe}{ed,to,goo}
% % \icmlauthor{Aaoeu Iasoh}{goo}
% % \icmlauthor{Buiui Eueu}{ed}
% % \icmlauthor{Aeuia Zzzz}{ed}
% % \icmlauthor{Bieea C.~Yyyy}{to,goo}
% % \icmlauthor{Teoau Xxxx}{ed}
% % \icmlauthor{Eee Pppp}{ed}
% \end{icmlauthorlist}

% \icmlaffiliation{to}{Graduate School of Information Science and Technology,
% The University of Tokyo, Tokyo, Japan}
% % \icmlaffiliation{goo}{Googol ShallowMind, New London, Michigan, USA}
% % \icmlaffiliation{ed}{School of Computation, University of Edenborrow, Edenborrow, United Kingdom}

% \icmlcorrespondingauthor{Cieua Vvvvv}{c.vvvvv@googol.com}
% % \icmlcorrespondingauthor{Eee Pppp}{ep@eden.co.uk}

% % You may provide any keywords that you
% % find helpful for describing your paper; these are used to populate
% % the "keywords" metadata in the PDF but will not be shown in the document
% \icmlkeywords{\Poincare  embeddings, Riemannian geometry, graph embeddings}

% \vskip 0.3in
% ]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

%\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
\printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.

